Understanding the Security Benefits and Overheads of Emerging Industry Solutions to DRAM Read Disturbance

We present the first rigorous security, performance, energy, and cost analyses of the state-of-the-art on-DRAM-die read disturbance mitigation method, Per Row Activation Counting (PRAC), described in JEDEC DDR5 specification's April 2024 update. Unlike prior state-of-the-art that advises the memory controller to periodically issue refresh management (RFM) commands, which provides the DRAM chip with time to perform refreshes, PRAC introduces a new back-off signal. PRAC's back-off signal propagates from the DRAM chip to the memory controller and forces the memory controller to 1) stop serving requests and 2) issue RFM commands. As a result, RFM commands are issued when needed as opposed to periodically, reducing RFM's overheads. We analyze PRAC in four steps. First, we define an adversarial access pattern that represents the worst-case for PRAC's security. Second, we investigate PRAC's configurations and security implications. Our analyses show that PRAC can be configured for secure operation as long as no bitflip occurs before accessing a memory location 10 times. Third, we evaluate the performance impact of PRAC and compare it against prior works using Ramulator 2.0. Our analysis shows that while PRAC incurs less than 13% performance overhead for today's DRAM chips, its performance overheads can reach up to 94% for future DRAM chips that are more vulnerable to read disturbance bitflips. Fourth, we define an availability adversarial access pattern that exacerbates PRAC's performance overhead to perform a memory performance attack, demonstrating that such an adversarial pattern can hog up to 94% of DRAM throughput and degrade system throughput by up to 95%. We discuss PRAC's implications on future systems and foreshadow future research directions. To aid future research, we open-source our implementations and scripts at https://github.com/CMU-SAFARI/ramulator2.

==> hpca-template.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%% -- DO NOT MODIFY -- %%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\author{
  \ifdefined\hpcacameraready
    \IEEEauthorblockN{\hpcaauthors{}}
      \IEEEauthorblockA{
        \hpcaaffiliation{} \\
        \hpcaemail{}
      }
  \else
    \IEEEauthorblockN{\normalsize{HPCA \hpcayear{} Submission
      \textbf{\#\hpcasubmissionnumber{}}} \\
      \IEEEauthorblockA{
        Confidential Draft \\
        Do NOT Distribute!!
      }
    }
  \fi 
}

% Heading and footer for title page
\fancypagestyle{camerareadyfirstpage}{%
  \fancyhead{}
  \renewcommand{\headrulewidth}{0pt}
  \fancyhead[C]{
    \ifdefined\aeopen
    \parbox[][12mm][t]{13.5cm}{\hpcayear{} IEEE International Symposium on High-Performance Computer Architecture (HPCA)}    
    \else
      \ifdefined\aereviewed
      \parbox[][12mm][t]{13.5cm}{\hpcayear{} IEEE International Symposium on High-Performance Computer Architecture (HPCA)}
      \else
      \ifdefined\aereproduced
      \parbox[][12mm][t]{13.5cm}{\hpcayear{} IEEE International Symposium on High-Performance Computer Architecture (HPCA)}
      \else
      \parbox[][0mm][t]{13.5cm}{\centering
      \hpcayear{} IEEE International Symposium on High-Performance Computer Architecture (HPCA)\\
      \textcolor{blue}{\textbf{Version~\theversion{}~---~\today, \ampmtime{}}}}
    \fi 
    \fi 
    \fi 
    \ifdefined\aeopen 
      \includegraphics[width=12mm,height=12mm]{ae-badges/open-research-objects.pdf}
    \fi 
    \ifdefined\aereviewed
      \includegraphics[width=12mm,height=12mm]{ae-badges/research-objects-reviewed.pdf}
    \fi 
    \ifdefined\aereproduced
      \includegraphics[width=12mm,height=12mm]{ae-badges/results-reproduced.pdf}
    \fi
  }
  %\fancyfoot[L]{\hpcapubid{} \copyright \hpcayear{} IEEE}
  \fancyfoot[C]{}
}
% Heading and footer for remaining pages
\fancyhead{}
\renewcommand{\headrulewidth}{0pt}
%\fancyhead[C]{\hpcayear{} IEEE International Symposium on
% High-Performance Computer Architecture (HPCA)}

% \renewcommand{\citepunct}{,\penalty\citepunctpenalty\,} \renewcommand{\citedash}{--}

\makeatletter
\def\bstctlcite{\@ifnextchar[{\@bstctlcite}{\@bstctlcite[@auxout]}}
\def\@bstctlcite[#1]#2{\@bsphack
 \@for\@citeb:=#2\do{%
   \edef\@citeb{\expandafter\@firstofone\@citeb}%
   \if@filesw\immediate\write\csname #1\endcsname{\string\citation{\@citeb}}\fi}%
 \@esphack}
\makeatother


  


==> sections/a_latencyevaluation.tex <==
\section{\agy{1}{Memory Access Latency Evaluation}}
\agycomment{1}{I am ok by removing the latency analysis to open up space for showing how much the attack can degrade performance. We can use it to motivate BreakHammer. Latency analysis can stay in the appendix.}
Figure~\ref{fig:benign_latency} presents the memory \agy{1}{access} latency \agy{1}{distribution} of the evaluated \agy{1}{read disturbance} mitigation mechanisms \agy{1}{(color-coded)} where the x-axis shows the percentile \agy{1}{of memory accesses and} the y-axis shows the memory \agy{1}{access} latency. 
% the black dashed line identifies the no mitigation baseline, and each colored continuous line identifies a different \gls{nrh} value.
\agycomment{1}{How come we have memory accesses that complete in less than 10ns? Do we include cache hits here? Even row buffer hits should take longer...}
\ouscomment{1}{Yes, the analysis includes any request that leaves the core. So, it also includes cache hits.}
\agycomment{1}{Can we also add horizontal grid lines for 1, 5, 10, 50, 100, 500, 1000, 5000, and 10000ns?}

\begin{figure}[h]
\centering
\includegraphics[width=\linewidth]{figures/_fourcore_benign_latency.pdf}
\caption{Memory latency impact of evaluated RowHammer mitigation mechanisms on four-core benign workloads.}
\label{fig:benign_latency}
\end{figure}

\ous{5}{We make \param{four} observations from \figref{fig:benign_latency}.
First, PARA incurs the most average memory latency overhead by \param{2.4}x at $\nrh{} = 64$.
Second, \gls{prac}-4, \gls{prac}-Ideal, and Graphene incur the least average memory latency overhead by \param{7.9}\%, \param{24.4}\%, and \param{11.2}\%, respectively at $\nrh{} = 64$.
Third, \gls{prfm}'s average memory latency overhead increases by \param{16.8}x when $\nrh{}$ decreases from 64 to 16. 
Fourth, \gls{prfm} and PARA incur the most average memory latency overhead by \param{10.5}x and \param{7.1}x, respectively at $\nrh{} = 16$.

Based on these observations we conclude that 1) \gls{prac} performs comparable to prior state-of-the-art defense mechanisms, and 2) \gls{prfm} incurs significant latenc overheads as \gls{nrh} decreases, to the point where \gls{prfm} is only comparable to PARA.}

==> sections/b_performanceattack.tex <==
\section{Extended Performance Degradation Attack Analysis}

\ous{1}{We analyzed the \gls{prac}'s secure configurations (\secref{sec:configurationandsecurity}) and the performance implications of these configurations on benign workloads (\secref{subsec:perfandstorageeval}).
While these configurations provide robust execution against read disturbance attacks, an attacker can take advantage of \gls{prac} mechanisms to degrade the system throughput by triggering as many preventive actions as possible in quick succession.
In this section, we 1) analyze the theoretical maximum downtime of a system protected by \gls{prac} mechanisms, and 2) run cycle-accurate simulations on Ramulator2~\cite{luo2023ramulator2} with an attacker present to show the throughput implications of our calculation in a realistic system.}

\ouscomment{1}{This can also be approximated with (time to refresh) / (time to trigger + time to refresh)}
\head{Theoretical Analysis}
\ous{1}{For our analysis we assume that
1) \gls{prac} mechanisms refresh all ranks within a module within a recovery period, and
2) protected systems use \gls{rfmab} command to refresh aggressor rows.}\footnote{\ous{1}{Current DDR5 specification~\cite{jedec2024jesd795c} allows \gls{prfm} system to use \gls{rfmsb} instead of \gls{rfmab} to reduce the number of banks unavailable during a preventive refresh. However, an attacker can intelligently hammer many banks across bank groups in parallel, and trigger multiple \gls{rfmsb} commands in quick succession that disable access to all banks. Therefore, we choose \gls{rfmab} to simplify our analysis.}}

\ous{1}{To estimate the throughput loss of a system, we analyze the maximum possible duration taken by preventive actions within a \gls{trefw}.
We perform our analysis in \param{four} steps by calculating:
1) the available time after DRAM refreshes ($t_{available}$),
2) the period to triggering a preventive action ($T_{attack}$),
3) the maximum time consumable by preventive actions within a refresh window ($t_{prevent}$), and
4) the throughput lost due to preventive actions ($t_{prevent}$/$t_{available}$), respectively.
The memory controller issues a \gls{ref} command every \gls{trefi} that takes \gls{trfc}.
Therefore, $t_{available} = \trefw - \trfc\times(\trefw/\trefi)$.
We continue our analysis for \gls{prfm} and \gls{prac} in their respective sections.}

\subhead{\gls{prfm}}
\ous{1}{An attacker can trigger an \gls{rfmab} command every \gls{rfmth} activations targeting a single bank.
\gls{rfmth} activations take $\rfmth\times\trc$ and the \gls{rfmab} command takes \gls{trfm}, which yields $T_{attack}$ = $\rfmth\times\trc$ + $\trfm$.
It is possible to trigger $t_{available}/T_{attack}$ \gls{rfmab} commands within a refresh window.
Therefore, $t_{prevent}$ is calculated as $\trfm\times(t_{available}/T_{attack})$.
As an example, we configure \gls{rfmth} as \param{6} against an \gls{nrh} of \param{64}.
% 16 GB 3200AN (all ns)
% tRC = 47
% tREFW = 32000000
% tREFI = 3900
% tRFC = 295
% tRFM = 295
% t_avail = 32000000 - 295*(32000000/3900) = 29579487.1795
% T_attack = 6 * 47 + 295 = 577
% t_prevent = 295 * 29579487.1795 / 577 = 15122961.4
% t_prevent / t_avail = 15122961.4 / 29579487.1795 = 0.511265165
By plugging the \param{DDR5-3200AN}~\cite{jedec2024jesd795c}\ouscomment{1}{i must double check this} timing preset, we obtain the $t_{available}$, $T_{attack}$, and $t_{prevent}$ as \param{$\approx$29.58ms}, \param{577ns}, and \param{$\approx$15.12ms}, respectively.
Based on these values, we observe that an attacker can \emph{theoretically} consume \param{$\approx$51\%} of available system throughput by triggering \gls{prfm} preventive actions.}

\subhead{\gls{prac}}
\ous{1}{We assume that a back-off signal is triggered when a row activation counter reaches \gls{aboth}, i.e., we assume a 100\% back-off trigger quantization.
We observe that row activations between recovery periods still increment the counters of aggressor rows.
An attacker can exploit this observation by hammering a single row, and trigger a back-off every \gls{aboth} activations.
\gls{aboth} activations take $\aboth\times\trc$ and the recovery period takes $\bonrefs\times\trfm$, which yields $T_{attack}$ = $\aboth\times\trc$ + $\bonrefs\times\trfm$.
Note that $T_{attack}$ always exceeds \gls{taboact} + \gls{tbodelay}, i.e., the minimum time between consecutive recovery periods, as \gls{prac} is \emph{not} safe for $\nrh$ values lower than \param{10}.
Therefore an attacker can trigger $t_{available}/T_{attack}$ recovery periods within a refresh window.
By factoring the $\bonrefs$ for each recovery, we obtain $t_{prevent}$ = $\bonrefs\times\trfm\times(t_{available}/T_{attack})$.
We respectively configure \gls{aboth}, $\bonrefs$, and $\bonacts$ as \param{57}, \param{4}, and \param{4} against an \gls{nrh} of \param{64}.
% 16 GB 3200AN (all ns)
% tRC = 52 (increased due to PRAC)
% tREFW = 32000000
% tREFI = 3900
% tRFC = 295
% tRFM = 350 (increased due to PRAC)
% t_avail = 32000000 - 295*(32000000/3900) = 29579487.1795
% T_attack = 228 * 52 + 4 * 350 = 4144
% t_prevent = 4 * 350 * 29579487.1795 / 4144 = 9993069.99
% t_prevent / t_avail = 9993069.99 / 29579487.1795 = 0.337837838
By plugging the \param{DDR5-3200AN}~\cite{jedec2024jesd795c} timing preset, we obtain the $t_{available}$, $T_{attack}$, and $t_{prevent}$ as \param{$\approx$29.58ms}, \param{3859ns}, and \param{$\approx$9.04ms}, respectively.
Based on these values, we observe that an attacker can \emph{theoretically} consume \param{$\approx$31\%} of available system throughput by triggering back-offs.}

\head{Simulation Results}
\ous{1}{To further understand the throughput degradation an attacker could incur in a system, we create \param{60} \param{four}-core workload mixes of varying memory intensities where a single core is malicious. It is \emph{not} possible to reliably open and close a single row with load and store instructions. Therefore, our attacker selects \param{8} rows from \param{4} banks and hammers them.}\footnote{\ous{1}{We experimentally found these values to yield the highest overhead against \gls{prfm} and \gls{prac} mechanisms for our system configuration. We will also open-source our attacker trace generator with the rest of our implementation to support reproducibility and easy adoption of these new features.}}

\ous{1}{\figref{fig:attack_scaling_appendix} presents the throughput overheads of the evaluated \agy{2}{read disturbance} mitigation mechanisms as \gls{nrh} decreases when an attacker is present. Here, the x-axis shows the different \gls{nrh} values, the y-axis shows the throughput loss of each workload normalized to the baseline system with \agy{2}{\emph{no} read disturbance} mitigation, and each bar identifies a different \agy{2}{read disturbance} mitigation mechanism.}

\begin{figure}[h]
\centering
\includegraphics[width=\linewidth]{figures/_fourcore_attack_scaling.pdf}
\caption{Energy impact of evaluated \agy{2}{read disturbance} mitigation mechanisms on four-core benign workloads.}
\label{fig:attack_scaling_appendix}
\end{figure}

\ous{1}{From \figref{fig:attack_scaling_appendix}, we observe that at $\nrh = 64$, \gls{prfm} and \gls{prac} incur a throughput loss of \param{44.0}\% and \param{15.1}\%, respectively.
While our \gls{prfm} results are similar to the analysis, \gls{prac} is not.
We attribute this discrepancy to \emph{not} being able to hammer a single row consistently in a real system.
\gls{prfm} is not affected by this problem as it does \emph{not} precisely track rows.
Therefore, it is enough for our attacker to create row conflicts in a bank and generate as many \gls{act} commands as possible.}

==> sections/stale.analysis.tex <==
\section{Attack Definition and Security Analysis}
\label{sec:analysis}

For our analysis, we assume that 1) the DRAM chips have perfect tracking, i.e., \gls{prac}, 2) the \gls{rfm} command always refreshes the victims of a row with the maximum activation counter, 3) the attacker can reverse engineer the logical to physical DRAM address translation, and 4) an attacker can deduce which row is refreshed internally for tie-breaker refreshes (i.e., an \gls{rfm} refresh between rows with the same activation counter).

We make \param{two} important observations from our trivial configuration analysis where the system designer chooses $\rfmth = \nrh - 1$.

\obs{obs:decoy}{An attacker can choose a set of rows as \emph{\agy{0}{decoy}} rows and boost other rows' maximum achievable activation counts.}

\obs{obs:ref}{An attacker should equally distribute their activations to the \emph{\agy{0}{decoy}} and \emph{real} attacker rows. By doing so, the attacker obtains new sets of rows with increasing activation counts.}

Based on these preliminary observations, we mathematically define our attack as \param{two} recurrences in Takeaway~\ref{tak:decoydef} and \ref{tak:recdef}.

\takeaway{tak:decoydef}{Selecting a set of rows of non-zero size $B_{i}$ with a minimum activation counters across these rows of $A_{i}$, and activating each row in $B_{i}$ once yields a new set of rows of size $B_{i+1}$ with activation counts $A_{i+1}$, where $B_{i+1} \leq B_{i}$ and $A_{i+1} = A_{i}+1$.}

\obs{obs:decoydefrec}{An attacker can start with an arbitrary set of rows of size $B_{0}$ and recursively attack the resulting sets of rows $B_{1}, B_{2}, ...\ B_{n}$ to achieve the increasing row activations of $A_{1}, A_{2}, ...\ A_{n}$.}

\obs{obs:decoydefatk}{A cold attack that starts with rows $B_{0}$ with $A_{0} = 0$ always has $A_{i} = i$ for all $i$ where $B_{i} > 0$.}

\takeaway{tak:recdef}{We know that i) each \gls{rfmth} activations cause an \gls{rfm} command, and ii) an attacker must perform $B_{k}$ activations to increase each row counter in the set by one to obtain $B_{k+1}$.}

\begin{equation}
\label{eqn:recinit}
B_{k+1} = B_{k} - \Bigl\lfloor
\frac{
R_{k} + B_{k}
}{
RFM_{th}
} \Bigr\rfloor
\end{equation}

Here, $R_{k}$ denotes the bank activation counter at the start of step $k$. We can sum the total activations from the initial state and avoid introducing the recurrence $R$ to our calculations.
By doing so, the size of the remaining rows at step $i$ ($B_{i}$) can be found with Equation~\ref{eqn:recdef}. Here, $B_{0}$ is the number of initial rows with no assumed activation counters (i.e., $A_{0} = 0$). Note that the $A_{0} = 0$ assumption simplifies our analysis per Observation~\ref{obs:decoydefatk}.

\begin{equation}
\label{eqn:recdef}
B_{i} = B_{0} - \Bigl\lfloor
\frac{
\sum_{k=0}^{i-1} B_{k}
}{
RFM_{th}
} \Bigr\rfloor
\end{equation}

Each row in a DRAM module is refreshed periodically independent of their activation rates to prevent data loss against retention.
Therefore, for a system to be secure against RowHammer bitflips under \gls{rfm} protection, the \gls{rfmth} should be selected such that an attacker should never be able to choose $B_{0}$ large enough to reach a $B_{i} > 0$ where $i \geq \nrh{}$.

\obs{obs:refduration}{Each row in a DRAM module is refreshed every \gls{trefw}.
This operation is performed by issuing a \gls{ref} command every \gls{trefi} and this command takes \gls{trfc} to complete.
The \gls{dallref} can be found with Equation~\ref{eqn:allref}.

\begin{equation}
\label{eqn:allref}
\dallref = \frac{\trefw{}}{\trefi{}} * \trfc
\end{equation}}

% \obs{obs:maxrfm}
{An \gls{rfm} command is triggered for every \gls{rfmth} activations and this command takes \gls{trfm} to complete.
We can access a bank as fast as \gls{trc}.
Therefore, \gls{trfmperiod} can be found with Equation~\ref{eqn:rfmperiod}.

\begin{equation}
\label{eqn:rfmperiod}
\trfmperiod = \rfmth * \trc + \trfm
\end{equation}

Given \gls{trfmperiod}, we calculate \gls{maxrfm} with Equation~\ref{eqn:maxrfm}.

% There is a syntax error somewhere here
% \begin{equation}
% \label{eqn:maxrfm}
% \maxrfm = \frac{\trefw - \dallref}{\trfmperiod}
% \end{equation}}

\takeaway{tak:maxact}{Based on Observations~\ref{obs:refduration} and~\ref{obs:maxrfm}, we derive the \gls{maxact} in Equation~\ref{eqn:maxact}.

\begin{equation}
\label{eqn:maxact}
\maxact = \maxrfm * \rfmth
\end{equation}

We can further unroll this equation to obtain it in terms of primitives, which yields Equation~\ref{eqn:maxactsimp}.

\begin{equation}
\label{eqn:maxactsimp}
\maxact = \frac{\trefw - \frac{\trefw}{\trefi} * \trfc}{\rfmth * \trc + \trfm} * \rfmth
\end{equation}}

An attack can only trigger a bitflip if it can reach $B_{\nrh{}} > 0$ within a refresh window. We formally define the security requirement of \gls{rfm} in Takeaway~\ref{lem:rhsecure}.

\takeaway{lem:rhsecure}{An \gls{rfm} protected system is secure against RowHammer bitflips if at least \param{one} of the \param{two} following conditions are true:
\begin{enumerate}
    \item $B_{\nrh{}} = 0$
    \item $\sum_{k=0}^{N_{RH}-1} B_{k} > \maxact$
\end{enumerate}}

Based on Takeaway~\ref{lem:rhsecure} we perform an analysis of the maximum steps possible under a system with \gls{rfm} protection for varying \gls{rfmth} configurations and initial row set sizes. Figure~\ref{fig:rfmkiller} presents the results of our analysis where the x-axis shows the different $\rfmth{}$ values, the y-axis shows the maximum achievable step $i$ where $B_{i} > 0$, and each bar identifies a different starting row set size ($B_{0}$).

% \begin{figure}[h]
% \centering
% \includegraphics[width=\linewidth]{figures/rfmkilleranalplot.pdf}
% \caption{Maximum possible activations on a row achievable with related to initial row set sizes and $\rfmth$.}
% \label{fig:rfmkiller}
% \end{figure}

We make \param{N} observations from Figure~\ref{fig:rfmkiller}.
First, configurations with $\rfmth < 6$ prevent bitflips even at a very low $\nrh=64$ against all $B_{0}$ as the necessary number of activations to reach $B_{\nrh}$ is greater than $\maxact$.
Second, the maximum $\rfmth$ value of \param{80}\footnote{
\gls{rfm} commands can be post-poned until the bank activation counter reaches 10x \gls{rfmth} in the standard. However, once this threshold is reached an \gls{rfm} command needs to be issued every \gls{rfmth}.}
defined in JEDEC DDR5 specitifaction~\cite{jedecddr5} does not provide sensitive configuration to systems with $\nrh > 512$.

\subsection{Extension to Alert Back-Off Protocol}
\label{sec:aboanalysis}

The recently introduced Alert Back-Off Protocol~\cite{jedecddr5} allows the DRAM module to request extra time from the memory controller to perform refresh management operations. With the \gls{abo} protocol, the memory controller continues operation for a set duration ($tABO_{ACT}$) before the recovery period and has a row activation budget (e.g., \param{4} ACTs) after the recovery period, where the DRAM module \emph{cannot} make another \gls{abo} request.

We extend our analysis to determine safe threshold configurations of the \gls{abo} protocol, such that an attacker \emph{cannot} activate a row enough times to induce a bitflip. We make \param{two} observations. First, we highlight the attack opportunities present in the protocol. Second, we explain how our \gls{rfm} security analysis can be extended to \gls{abo}.

\obs{obs:pracoppor}{There are \param{two} opportunities an attacker can exploit to increase their attack efficiency.
First, the module does not request an \gls{abo} until one of the rows reaches the \gls{aboth}. The attack can use this period to bring up attacker and decoy rows to some activation level.
Second, several row activations must be scheduled between consecutive \gls{abo}s. The attack can use this period to continue the wave attack.}

\obs{obs:rfmtoprac}{From Observation~\ref{obs:pracoppor}, an attacker can initially start with a set of rows with activation counts $\aboth{}-1$. Following this initialization, the first-row activation will cause an \gls{abo}, and every \param{$\aboact{}+\abodelay{}$} activations will be followed by \param{$\aboact{}$} refreshes. Based on our observation, we map this pattern to our earlier analysis where $\rfmth{}=\aboact{}+\abodelay{}$ and each RFM removing $\aboact{}$ rows.}

Based on Observation~\ref{obs:rfmtoprac} we derive the number of remaining rows at attack step $i$ ($B_i$) with Equation~\ref{eqn:pracstep}.

\begin{equation}
\label{eqn:pracstep}
B_{i} = B_{0} - \aboact{} * \Bigl\lfloor
\frac{
\sum_{k=0}^{i-1} B_{k}
}{
\aboact{} + \abodelay{}
} \Bigr\rfloor
\end{equation}

\takeaway{tak:pracsecure}{An \gls{abo} protected system is secure against RowHammer bitflips if at least \param{one} of the \param{two} following conditions are true:
\begin{enumerate}
    \item $B_{\nrh{}-\aboth{}+1} = 0$
    \item $(\sum_{k=0}^{\nrh{}-\aboth{}} B_{k}) + (\aboth{}-1 * B_0) > \maxact$
\end{enumerate}
The first condition states that no initial decoy row size will allow an attacker to perform \gls{nrh} activations on a row. As the attacker initializes each starting row, we reduce the necessary attack step to reach by $\aboth{}-1$.
The second condition states that even if a starting row size allows $\nrh{}$ activations on a single row, the necessary activations to initialize these rows and perform the wave attack should fit into a refresh window.}

\subsection{Under Attack}

\begin{figure}[h]
\centering
\includegraphics[width=\linewidth]{figures/_fourcore_attack_scaling.pdf}
\caption{Attacker performance}
\label{fig:pracanalysis}
\end{figure}

\begin{figure}[h]
\centering
\includegraphics[width=\linewidth]{figures/_fourcore_attack_energy.pdf}
\caption{Attacker energy}
\label{fig:pracanalysis}
\end{figure}

\begin{figure}[h]
\centering
\includegraphics[width=\linewidth]{figures/_fourcore_attack_latency.pdf}
\caption{Attacker latency}
\label{fig:pracanalysis}
\end{figure}

